Conditionally Identifiable Latent-Environment Modeling for Out-of-Distribution Recommendation

Out-of-distribution (OOD) recommendation is vulnerable to preference shifts induced by a latent environment. Existing methods can infer latent states from logged interactions, yet the statistical meaning of the latent environment and its effect on preference remain underdetermined. We formulate this task as conditionally identifiable risk-aware recommendation (CI-RR) and propose Conditionally Identifiable Latent-Environment Recommendation (CILER). CILER uses a user-conditioned exponential family to model the latent environment and a feature-indexed polynomial to specify how it changes preference. It predicts by marginalizing item probabilities over the inferred environment distribution. Under sufficient variation, correct specification, and decoder regularity, CILER identifies the environment-sensitive representation up to the stated equivalence class. We further bound excess deployment log-risk by environment-inference error. Controlled studies test the observable consequences of sufficient variation and model specification. Experiments on three datasets show that CILER improves all twelve OOD ranking metrics under feature, temporal, and geographical shifts within shared support.

==> graphicalabstract.tex <==
% Graphical abstract -- Neurocomputing submission
\begin{graphicalabstract}
\includegraphics[width=1\textwidth]{polyfig/FRAMEWORK.pdf}
\end{graphicalabstract}


==> highlights.tex <==
% Highlights -- Neurocomputing submission
% Three to five bullet points, each at most 85 characters including spaces.
\begin{highlights}
\item Latent-environment identifiability becomes a requirement for OOD recommendation.
\item CILER infers a user-conditioned latent environment from logged interactions alone.
\item Sufficient context variation identifies the environment-sensitive representation.
\item Environment marginalization bounds excess deployment risk by inference error.
\item CILER leads all twelve OOD metrics and lifts Recall@100 by 25.6\% on Meituan.
\end{highlights}

